Partial Order Resolution of Event Logs for Process Conformance Checking

While supporting the execution of business processes, information systems record event logs. Conformance checking relies on these logs to analyze whether the recorded behavior of a process conforms to the behavior of a normative specification. A key assumption of existing conformance checking techniques, however, is that all events are associated with timestamps that allow to infer a total order of events per process instance. Unfortunately, this assumption is often violated in practice. Due to synchronization issues, manual event recordings, or data corruption, events are only partially ordered. In this paper, we put forward the problem of partial order resolution of event logs to close this gap. It refers to the construction of a probability distribution over all possible total orders of events of an instance. To cope with the order uncertainty in real-world data, we present several estimators for this task, incorporating different notions of behavioral abstraction. Moreover, to reduce the runtime of conformance checking based on partial order resolution, we introduce an approximation method that comes with a bounded error in terms of accuracy. Our experiments with real-world and synthetic data reveal that our approach improves accuracy over the state-of-the-art considerably.

==> sections/modelselection.tex <==

Having defined various behavioral models for partial order resolution, a key 
concern is the selection of the most appropriate model for a particular 
dataset. 
As a basis for such a selection, it should be noted that the models provide a 
trade-off between the \textit{strictness} of the notion of behavioral 
regularity that is employed, and the \textit{selectivity} of the model with 
respect to an event log. 
%For instance, the 
%trace equivalence model is the strictest as it derives probabilities only from 
%fully identical traces. Yet, the number of traces for partial order resolution 
%may severely be limited. 
Below, we first discuss this strictness of models in more detail 
(\autoref{sec:behavioralstrictness}). Based on this discussion, we elaborate on 
measures that guide the selection of a model for a given log 
(\autoref{sec:selectionmeasures}) and the actual selection 
(\autoref{sec:selection}).



\subsection{Strictness of Behavioral Models}
\label{sec:behavioralstrictness}
 
The proposed behavioral models can be ordered in terms of their strictness, the 
trace equivalence model is stricter than the N-gram one, which is stricter than 
the weak order one. 
%Ranging from most to least restrictive, this ordering is:
% 
%  \textit{trace equivalence} $>$ \textit{N-gram} $>$  \textit{weak order}. 
Also, for N-gram models, the larger $N$, the stricter the model.
%, e.g. a 4-gram model is more restrictive than a 2-gram model. 
 
The use of stricter models can be important in order to identify long distance 
dependencies among events, as illustrated with the following traces:

\vspace{0.5em}
\begin{tabular}{rl}
		$\sigma_3$ &  $ = \langle \{b\}, \{c\}, \{d\}, \{e, f\} \rangle $ \\
		$\sigma_4 =  \sigma_5 =\sigma_6 = \sigma_7 $ & $ = \langle \{a\}, \{c\}, 
		\{d\}, \{e\}, \{f\}\rangle$ \\ 
		$\sigma_8 = \sigma_9 $  & $= \langle \{b\}, \{c\}, 
		\{d\}, \{f\}, \{e\}\rangle$ \\ 
	
\end{tabular} 
	
	\vspace{0.5em}
There is one uncertain trace, $\sigma_3$, with resolutions $\varphi_{3}=\langle 
b,c,d,e,f\rangle$ and 
$\varphi_{4}=\langle b,c,d,f,e\rangle$, whereas all remaining traces are 
certain. Applying a less strict model (N-gram with $N<4$ or weak 
order), there are four traces that support a resolution 
in which $e$ precedes $f$, meaning that there is 
more evidence for $\varphi_3$ than for $\varphi_4$ and it holds 
$P(\varphi_{3})>P(\varphi_{4})$.

However, note that all traces that provide evidence for $\varphi_3$, i.e., traces $\sigma_4$ to $\sigma_7$, start with event $a$. By contrast, the traces that support resolution $\varphi_4$ always start with event $b$. This is important, because it hints at a dependency between the 
occurrence of $a$ or $b$, on the one hand, and the order in which $e$ and $f$ occur, on the other. Such a long 
distance dependency, from 
the first event to the fourth and fifth event, is only recognized in a 
strict behavioral model, such as the N-gram model, here with $N\geq 4$, or the 
trace equivalence model.
%, but would be missed by less restrictive behavioral models. 

This example suggests a preference for selecting strict behavioral models. 
However, given that stricter models imply higher selectivity, we strive for the 
selection of the strictest model that still provides sufficient evidence for 
partial order resolution. Whether a model is sufficient may be quantified along 
several dimensions, which we capture by \textit{selection measures}, as 
discussed next.

\subsection{Selection Measures}
	\label{sec:selectionmeasures}

To guide the selection of a behavioral model for a given event log, we define 
three selection measures: (i) log coverage, (ii) resolution support, and (iii) 
uncertainty ratio.

\smallskip
\noindent \textbf{Log Coverage.} The \textit{log coverage} is the fraction of 
uncertain traces in a log, for which a behavioral model provides insights into 
its resolution, i.e., for which the model provides a non-zero probability for 
at least one resolution. 
%For the trace equivalence model, e.g., this holds 
%true only if at least one resolution corresponds to a certain trace in the 
%log. 
	
To formalize this measure, we write $\Sigma_{unc.} = \{ \sigma \in \Sigma\ |\  
|\Phi(\sigma)| > 1 \}$ for all uncertain traces. Let $P_M(\varphi)$ be the 
probability assigned to a resolution $\varphi$ by a behavioral model $M$. Then, 
we define the coverage of behavioral model 
$M$ for event log $\Sigma$ as: 

\vspace{-.6em}
\footnotesize
\begin{equation}
\label{eq:coverage}
coverage(\Sigma, M) =  \frac{  |\{ \sigma \in \Sigma_{unc.}\ |\ \exists\ 
\varphi \in \Phi(\sigma) : P_M(\varphi) > 0    \}|  }{| \Sigma_{unc.}|}
\end{equation} 

\vspace{-.3em}
\normalsize
Having a high log coverage can be seen as a basic requirement for a selected 
behavioral model: if log coverage is low, the selected 
model will not be able to provide insights for a 
considerable number of traces. Yet, providing a satisfactory 
coverage does not necessarily imply that a model is actually 
suitable for a log. It is also important that a behavioral model 
computes probabilities on the basis of a sufficient amount of information, 	
 as captured by the following measures.

\smallskip
\noindent \textbf{Resolution support.} The \textit{resolution support} corresponds to the number of traces that 
supported the 
computation of probabilities for resolutions containing a specific type of 
uncertainty. 
Intuitively, when resolution support is high, probabilities are computed based 
on 
information from a large number of available traces. By contrast, low 
support indicates that the behavioral model may be overfitting, as only a 
few traces are considered. 	
Resolution support can be measured at various levels of detail. Primarily, we 
can quantify support on the trace level and the activity-pair level. 

We define a predicate $supp(\sigma, M, \varphi)$, denoting that for a given 
behavioral model $M$, the trace 
$\sigma$ provides evidence for a resolution $\varphi$. For instance, for the 
trace equivalence model $M_{TE}$, the predicate $supp(\sigma, M_{TE}, \varphi)$ 
only holds if $\sigma$ is a certain trace following the same event sequence as 
resolution $\varphi$. 
Based thereon, we define support on the trace level as:


\vspace{-.6em}
\footnotesize
\begin{equation}
	\label{eq:supporttracelevel}
	support(\sigma, M) = |\{ \sigma' \in \Sigma\ |\ \exists\ \varphi \in 
	\Phi(\sigma) : supp(\sigma', M, \varphi)                \}||
\end{equation} 

\vspace{-.3em}
\normalsize
Intuitively, we check for each trace $\sigma'$, if it 
provides support for any of the resolutions in $\Phi(\sigma)$. 

Next, we define support at the activity-pair level, which quantifies the amount 
of traces that are used by a model $M$ to resolve uncertainty between events 
corresponding to two activities, $x$ and $y$. To quantify this, we use 
$\Sigma_{unc.(x,y)}$ to denote the set of traces that contain uncertainty 
between events corresponding to activities $x$ and $y$, leading to the following definition of support:

\begin{equation}
\label{eq:supportpairlevel}
\begin{split}
support(\Sigma, M, x, &y) = \\ |\{ \sigma \in \Sigma\ |\  \exists\  \sigma' \in 
&\Sigma_{unc.(x,y)}, \varphi \in \sigma' :  supp(\sigma', M, 
\varphi)                \}|
	\end{split}
\end{equation} 

By considering both the coverage and support measures, we can provide a 
guarantee with respect to the ability of the 2-gram and weak order models to 
resolve uncertainty:

\begin{property}[Coverage Guarantee]
	\label{prop:coverageguarante}
	Given an event log $\Sigma$ and $M$ as either a 2-gram or a weak order 
	behavioral model, it holds that: For any pair of activities 
	$x, y$, for which there exists uncertainty in the event log, i.e., 
	$|\Sigma_{unc.(x,y)}| \geq 0$, if $support(\Sigma, M, x, y) \geq 1$, then 
	$coverage(\Sigma, M) = 1.0$.
\end{property}

This means that if there is at least some evidence for 
the resolution related to a pair of activities, the 
weak order and 2-gram model will resolve the uncertainty in all traces.
	
	
	
\smallskip
\noindent\textbf{Uncertainty ratio.} Finally, we introduce the 
\textit{uncertainty ratio} to capture the ratio between the resolution support and the 
amount of uncertainty that exists in an event log. By taking both of these 
factors into account, we conclude on the confidence to be put in the 
probabilities assigned by a behavioral model. 
	
To illustrate the importance of this ratio, consider two event logs $L_1$ and 
$L_2$ and some behavioral model $M$. Assume that both $L_1$ and $L_2$ contain 5 
traces that support the resolution of uncertainty between events $b$ and 
$c$, i.e., $support(L_1, M, b, c) = support(L_2, M, b, c) = 5$. Without further 
information, it may seem that $M$ is a suitable behavioral model to resolve 
uncertainty between these events for both logs. However, it may be the case 
that $L_1$ contains a single trace with uncertainty between $b$ 
and $c$, whereas $L_2$ contains 95 traces with uncertainty between these 
events. Then, for $L_2$, only 5 traces are used to resolve uncertainty in 95 
traces, so that there is a considerable risk that the model $M$ would 
overfit on the 5 traces. This risk is much lower for $L_1$, given that there 
are much more certain traces than uncertain ones for this particular type of 
uncertainty. To quantify this property, we introduce the $uncertaintyRatio$ 
measure as follows:

\vspace{-.6em}
\small
\begin{equation}
\label{eq:uncertaintyratio}
uncertaintyRatio(\Sigma, M, x, y) =  \frac{support(\Sigma, M, x, 
y)}{\Sigma_{unc.(x,y)}}
\end{equation} 

\vspace{-.3em}
\normalsize
The $uncertaintyRatio$ is used to determine the ratio between the amount of 
evidence that model $M$ can gather in a log $\Sigma$, for a particular pair of 
events, versus the amount of traces that require resolution of this type of 
uncertainty. 

Finally, to understand the ratio of support versus uncertainty at 
the log level, we can compute the uncertainty ratio for an entire event 
log as the average of the uncertainty ratios of all activity-pairs $x$, 
$y$ for which there exists uncertainty in the log.

%		\begin{equation}
%	\label{eq:uncertaintyratioavg}
%	uncertaintyRatio(\Sigma, M) =  \frac{support(\Sigma, M, x, y)}{\Sigma_{unc.(x,y)}} 
%	\end{equation} 
	
%	\todo{create equation}
	
\subsection{Selecting a Model based on the Measures}
\label{sec:selection}

The introduced measures enable conclusions on the appropriateness of a chosen 
behavioral model for an event log. The idea is to the select the strictest 
model, in order to be able to identify long-distance dependencies, for which 
the coverage is sufficiently high (e.g., $> 0.8$)  and the uncertainty ratio 
reasonably low (e.g., $< 0.2$). Conveniently, both of these requirements can be 
satisfied at the same time, given the relation between coverage and the 
uncertainty ratio. In particular, we can establish the following property:

\begin{property}[Coverage and Uncertainty Ratio.]
	\label{prop:coverageandratio}
	Given two behavioral models $M_1$ and $M_2$, where $M_1$ is more strict than $M_2$, then, for any event log $\Sigma$, $coverage(\Sigma, M_1) \leq coverage(\Sigma, M_2)$ and $uncertaintyRatio(\Sigma, M_1) \geq uncertaintyRatio(\Sigma, M_2)$. 
\end{property} 

Property~\ref{prop:coverageandratio} follows directly from the increase in the 
evidence that can be used for uncertainty resolution when a less strict 
behavioral model is selected. 
%Therefore, for a less strict model, coverage will either increase or remain 
%equal and, similarly, the uncertainty ratio will decrease or stay even. 
By using this property, moving from the trace equivalence model, through the 
N-gram model 
with decreasing $N$, to the weak order model, the $coverage$ and 
$uncertaintyRatio$ measures indicate when an 
appropriate abstraction level has been obtained. 


==> sections/scalability.tex <==

One of the key issues hindering the applicability of conformance checking 
techniques in industry is their computational 
complexity~\cite{vanderaalst2012replaying}. Therefore, the ability to obtain 
conformance checking results efficiently is of critical importance. In the 
context of this paper, the issue of complexity is particularly problematic, 
since order uncertainty exponentially increases the number of conformance 
checks that are required per trace. For instance, consider a 
partially ordered trace with a single uncertain event set. If this uncertain 
event set contains five events, already 120 conformance checks are required. 

To deal with this problem, we exploit the fact that resolutions with higher 
probabilities have a much greater impact on the final outcome of conformance checking than those with 
low probabilities. This means that considering the most likely order resolutions (instead of all possible ones) can be sufficient for obtaining 
reliable conformance checking results. Building on this insight, we introduce 
three approximation methods to reduce the runtime: 

\smallskip
\noindent
\textbf{Top-k selection}: A simple way of reducing the number of required 
conformance checks is to only conduct conformance checks for the \textit{k} 
most probable possible partial order resolutions. While this still requires to 
compute the probability of each possible order resolution according to the 
selected behavioral model, it dramatically reduces the number of required 
conformance  checks, keeping them to a predefined maximum of \textit{k} checks 
per trace. 

\smallskip
\noindent
\textbf{Probability-based cutoff}: An obvious disadvantage of top-k selection 
is that it does not consider the overall certainty that is provided by the 
selected resolutions. While a top-k selection with k=3 seems a reasonable 
for a trace with six resolutions, it might be unreasonable for a trace with 
hundreds of low-probability resolutions. Recognizing this, we introduce an alternative selection 
mechanism. The idea is to define a cutoff for the cumulative probability 
all considered resolutions need to have. For instance, starting with the most likely resolutions, we perform conformance checks until we have covered resolutions with a cumulative probability of 80\%.  In this way, we make sure that we take 
a sufficient number of resolutions into consideration. While this strategy does 
not allow us to fully estimate the number of conformance checks, it will still 
reduce the number considerably. 

\smallskip
\noindent
\textbf{Majority cutoff}: A strategy that reduces the number of required
conformance checks without the risk of drawing incorrect conclusions, is to 
check when the consideration of an additional partial order resolution can no 
longer change the overall conformance outcome, i.e., whether a trace is more likely to be conforming or non-conforming. This is the case once the cumulative probability of 
either conforming or non-conforming resolutions is higher than 
0.5. While this strategy may save less time than the strategies above 
(depending on the selected \textit{k} and cutoff), it provides more accurate 
results. 

The above introduced approximation methods provide a tradeoff between accuracy 
and runtime. It is, however, important to note that the error in accuracy can be well controlled
when using the probability-based cutoff. The majority cutoff even provides a guarantee. When the
majority cutoff is reached, then the conformance outcome, conforming or non-conforming, is identical to the outcome that would be obtained by checking every single resolution.
 
 



